Planetary-Mass Exosatellite Detected Around the Substellar Companion of a Star

Despite more than 6000 exoplanets being discovered to date, no satellite orbiting an exoplanet, an exomoon, has ever been confidently detected. While there are some candidates, they lack clear and convincing confirmation and remain controversial. Beyond the innate value of discovering new types of objects in the Universe, satellites can help give key insights into planet formation mechanisms and the dynamical evolution histories of their systems. In this work, we show strong evidence for the existence of satellites orbiting the directly-imaged brown dwarf companion CD-35 2722 B. We have applied radial velocity analysis, the same technique used to discover the first exoplanet around a Solar-type star, on spectra of this brown dwarf obtained with VLT/CRIRES+. We have found what appears to be the periodic signal induced by at least one orbiting satellite. This is the first time this technique has successfully produced evidence of satellites. We produce a strong detection of a satellite candidate with a minimum mass of 0.743 Jupiter masses and an orbital period of 169 days. The best-fitting model also includes a second, closer satellite with minimum mass of 0.277 Jupiter masses and a period of 87 days, although these parameters for this smaller satellite candidate are less certain. These periods would place them very near a 2:1 mean motion resonance, a phenomenon also seen in the Galilean moons of Jupiter. The discovery of these satellites will unlock many future avenues of study, including planet formation, system dynamics, and even the search for life in the Universe.

==> authors.tex <==
\author[0009-0004-5870-9562]{Kevin Hoy}
\affiliation{Instituto de Estudios Astrof\'isicos, Facultad de Ingenier\'ia y Ciencias, Universidad Diego Portales, Av.\ Ej\'ercito Libertador 441, Santiago, Chile}
\affiliation{European Southern Observatory, Alonso de C\'ordova 3107, Casilla 19, Santiago 19001, Chile}
\affiliation{Millennium Nucleus on Young Exoplanets and their Moons (YEMS)}

\author{0000-0002-5903-8316}{Alice Zurlo}
\affiliation{Instituto de Estudios Astrof\'isicos, Facultad de Ingenier\'ia y Ciencias, Universidad Diego Portales, Av.\ Ej\'ercito Libertador 441, Santiago, Chile}
\affiliation{Millennium Nucleus on Young Exoplanets and their Moons (YEMS)}

\author{Pablo ~A. Pe{\~n}a R.}
\orcidlink{0000-0002-8770-4398}
\institute{Instituto de Estudios Astrof\’isicos, Facultad de Ingenier\’ia y Ciencias, Universidad Diego Portales, Av. Ej\’ercito 441, Santiago, Chile}
\institute{Centro de Astrof\’isica y Tecnolog\’ias Afines (CATA), Casilla 36-D, Santiago, Chile}

\author{Jana K\¨ohler}
\affiliation{TLS Tautenburg, Sternwarte 5, 07778 Tautenburg, Germany}

\author{Silvano Desidera}
\affiliation{INAF-Osservatorio Astronomico di Padova, Vicolo Osservatorio 5, 35122 Padova, Italy}

\author{Raffaele Gratton}
\affiliation{INAF-Osservatorio Astronomico di Padova, Vicolo Osservatorio 5, 35122 Padova, Italy}

\author{Cecilia Lazzoni}
\affiliation{INAF, Astronomical Observatory of Padua, Vicolo dell'Osservatorio 5, I - 35122, Padua, Italy}

\author{Simon Petrus}
\affiliation{NASA-Goddard Space Flight Center, Greenbelt, MD 20771, USA}

\author{0000-0003-0650-5723}{Florian Rodler}
\affiliation{European Southern Observatory, Alonso de C\'ordova 3107, Casilla 19, Santiago 19001, Chile}

\author{0000-0002-3082-7266}{Jonathan Smoker}
\affiliation{European Southern Observatory, Alonso de C\'ordova 3107, Casilla 19, Santiago 19001, Chile}


\author{Valentina D'Orazi}
\affiliation{- Dept. of Physics, University of Rome Tor Vergata, via della Ricerca Scientifica 1, 00133, Rome, Italy}
\affiliation{INAF Osservatorio Astronomico di Roma, via Frascati 33, Monte Porzio Catone, 00040, Rome, Italy}


\author{Ilaria Carleo}
\affiliation{INAF -- Osservatorio Astrofisico di Torino, Via Osservatorio 20, I-10025, Pino Torinese, Italy}

\author[0009-0005-9376-7044]{Ilaria Giovannini}
\institute{Dipartimento di Fisica e Astronomia, Università degli Studi di Padova, Vicolo dell’Osservatorio 3, 35122 Padova, Italy}
\institute{Instituto de Estudios Astrof\’isicos, Facultad de Ingenier\’ia y Ciencias, Universidad Diego Portales, Av. Ej\’ercito 441, Santiago, Chile}
\affiliation{INAF-Osservatorio Astronomico di Padova, Vicolo Osservatorio 5, 35122 Padova, Italy}

